Finding Substitutable Binary Code By Synthesizing Adapters

Independently developed codebases typically contain many segments of code that perform same or closely related operations (semantic clones). Finding functionally equivalent segments enables applications like replacing a segment by a more efficient or more secure alternative. Such related segments often have different interfaces, so some glue code (an adapter) is needed to replace one with the other. We present an algorithm that searches for replaceable code segments at the function level by attempting to synthesize an adapter between them from some family of adapters; it terminates if it finds no possible adapter. We implement our technique using (1) concrete adapter enumeration based on Intel's Pin framework (2) binary symbolic execution, and explore the relation between size of adapter search space and total search time. We present examples of applying adapter synthesis for improving security and efficiency of binary functions, deobfuscating binary functions, and switching between binary implementations of RC4. We present two large-scale evaluations, (1) we run adapter synthesis on more than 13,000 function pairs from the Linux C library, (2) using more than 61,000 fragments of binary code extracted from a ARM image built for the iPod Nano 2g device and known functions from the VLC media player, we evaluate our adapter synthesis implementation on more than a million synthesis tasks . Our results confirm that several instances of adaptably equivalent binary functions exist in real-world code, and suggest that adapter synthesis can be applied for reverse engineering and for constructing cleaner, less buggy, more efficient programs.

==> IEEEtran/README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> adapter_results_partial.tex <==

\begin{table*}[]
\centering
\caption{adapters found within eglibc-2.19 using partial automation}
\label{table:libc-adapters-partial}
\begin{tabular}{ll}
\hline
target function $\leftarrow$ inner function                                                                                                                                                                      & adapter                                                                                   \\ \hline
isupper(1) $\leftarrow$ islower(1)                                                                                                                                                                            & \#0 + 32                                                                                  \\ \hline
islower(1) $\leftarrow$ isupper(1)                                                                                                                                                                            & \#0 - 32                                                                                  \\ \hline
killpg(1) $\leftarrow$ kill(1)                                                                                                                                                                            & -\#0, \#1                                                                                  \\ \hline
\end{tabular}
\end{table*}


==> overview.tex <==
\section{Overview} \label{sec:overview}
%Give an overview of adapters by using a motivating example. The most
%motivating example for now is the adapter between the isPalindrome
%variants, show either chartrans or simple+len here.

This section provides an overview of our adapter synthesis technique.
We begin with a motivating example. Consider the two implementations of the \textit{isPalindrome} predicate given in Listing \ref{lst:isPalindrome}.
The first implementation, \textit{isP1}, takes as input a pointer \textit{s} that points to the beginning of a string, and then computes another pointer \textit{p} that points to the end of that string using the C function \textit{strlen}. 
\textit{isP1} then checks that the characters pointed to
by \textit{s} and \textit{p} are equal as the two pointers are moved closer to each other. 
The second implementation of the \textit{isPalindrome} predicate, \textit{isP2}, takes as input a pointer to the beginning of a string and that string's length.
It then checks that the relevant corresponding characters are equal by indexing into the input string.

\lstinputlisting[caption={Two implementations of the
\textit{isPalindrome} predicate}, label={lst:isPalindrome}, style=nonumbers]{code_samples/simple-len.c}

Although \textit{isP1} and \textit{isP2} take a different number of arguments, they implement the same core functionality, and so we would like to consider them semantically-equivalent.
%
We justify their equivalence by the existence of an adapter that allows us to replace calls to \textit{isP1} with equivalent calls to \textit{isP2}.
%
An implementation of this adapter is given by the function \textit{adapted\_isP2}.
%
\textit{adapted\_isP2} has the same interface as \textit{isP1} and is implemented using a single call to \textit{isP2} with modified arguments.
%
Notice that it is not possible to adapt the interface of \textit{isP1} to \textit{isP2} because \textit{isP2} checks for the existence of a palindrome \textit{len} bytes long which need not always be equal to the length of the string beginning at \textit{start}.
%Notice that in this case it is also possible to replace calls to \textit{isP2} with adapted calls to \textit{isP1} using the function \textit{adapted\_isP2}. However, it is not always possible to construct adapters in both directions. 

This leads to the idea that the problem of comparing two functions for semantic equivalence is the same as the problem of finding an adapter between those two functions that allows one to be replaced by the other. 
%
This is the driving idea behind our approach to detecting semantically-equivalent code. 
%
To search for adapters between functions, we use a counterexample-guided search technique. 
%
Our algorithm, along with more examples of sematically-equivalent function pairs, is presented in Section~\ref{sec:adapter_synthesis}.

% TODO: it might be nice to add an example here of two functions whose return values match, but make different system calls or writes the memory (which means that they are not semantically-equivalent even though their input/return value behavior is the same)

But before moving on to the algorithm, we discuss some additional challenges of comparing the output of arbitrary functions for equivalence. 
One aspect of output equivalence is return value equivalence. 
In the example above this was straight-forward because both \textit{isP1} and \textit{isP2} only return either 0 or 1. 
But it may be the case that two functions with semantically-equivalent behaviors return values that have the same meaning, without having the same value.
Consider the semantically similar functions $f_1$ and $f_2$ shown in Listing \ref{lst:strcmp}.
While $f_1$ returns one if its argument strings are equal and zero otherwise, $f_2$ returns zero if its argument strings are equal and a non-zero value otherwise. 
$f_1$ can be adapted to $f_2$ only if its return value is changed to accommodate this difference in representation of string equality. 
\lstinputlisting[caption={Two C++ implementations for comparing strings}, label={lst:strcmp}, style=nonumbers]{code_samples/return-cmp-adapter.c}
%For example, the \textit{isupper} and \textit{islower} functions, which check whether a character is upper- or lower-case respectively, return the nonzero values 128 or 256 to idicate `true,' and 0 to indicate `false.'
%In this case the nonzero return values of both functions have the same semantic meaning without being exactly the equal. 
This idea of equivalent meaning (without equality) between return values motivates our use of adapters that apply to the inner function's return value as well as its input.

However, the return value alone does not capture a function's output behavior. 
%
We also need to consider side-effects such as system calls and modifications to memory.
%
One way to handle the system call component of side-effects is to only consider functions equivalent if they make the same sequence of system calls with equivalent arguments.
% 
Checking for equivalence of memory side-effects presents a greater challenge.
%
A shallow way to check for memory-based equivalence is to capture all writes made to memory by the target and inner functions and determine whether the same data is present at the same locations after both target and inner functions have finished execution.
%
But for a complete handling of memory side-effects, we also have to consider equivalence between writes to memory that write semantically equivalent values to the same location.
%
Further complications arise when we try to perform memory-based equivalence checking for functions that operate on pointer-rich data structures such as linked lists.
%Another complication is that when a function writes an address to memory, to properly compare that write with another function's write, we need to follow a chain of dereferenced addresses to get to non-address values. 


